Concury: A Fast and Light-weighted Software Load Balancer

A load balancer (LB) is a vital network function for cloud services to balance the load amongst resources. Stateful software LBs that run on commodity servers provides flexibility, cost-efficiency, and packet consistency. However current designs have two main limitations: 1) states are stored as digests which may cause packet inconsistency due to digest collisions; 2) the data plane needs to update for every new connection, and frequent updates hurt throughput and packet consistency. In this work, we present a new software stateful LB called Concury, which is the first solution to solve these problems. The key innovation of Concury is an algorithmic approach to store and look up large network states with frequent connection arrivals, which is succinct in memory cost, consistent under network changes, and incurs infrequent data plane updates. The evaluation results show that the Concury algorithm provides 4x throughput and consumes less memory compared to other LB algorithms, while providing weighted load balancing and false-hit freedom, for both real and synthetic data center traffic. We implement Concury as a prototype system deployed in CloudLab and show that the throughput of Concury on a single thread can reach 62.5% of the maximum capacity of two 10GbE NICs and that on two threads can reach the maximum capacity.

==> Makefile <==
All: Concury.pdf

%.pdf: %.tex *.tex *.bib Force
	rm -f *.aux
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' %.log) \
	do pdflatex $<; done

diff:
	git latexdiff --whole-tree --no-view --exclude-textcmd="section,subsection" -o diff.pdf SIGCOMM2019_init --

.PHONY: Figs Force diff

Figs:
	$(MAKE) -C Fig

Force:

